Minimally Constrained Stable Switched Systems and Application to Co-simulation

We propose an algorithm to restrict the switching signals of a constrained switched system in order to guarantee its stability, while at the same time attempting to keep the largest possible set of allowed switching signals. Our work is motivated by applications to (co-)simulation, where numerical stability is a hard constraint, but should be attained by restricting as little as possible the allowed behaviours of the simulators. We apply our results to certify the stability of an adaptive co-simulation orchestration algorithm, which selects the optimal switching signal at run-time, as a function of (varying) performance and accuracy requirements.

==> consensus.tex <==
\section{Optimal Solution in Consensus Algorithms}
\label{sec:consensus}

When switched systems possess an invariant polytope, the unstable cycles are easy to obtain \cite[Section~5]{Chevalier2015}.
In particular, the switched systems associated to the \emph{consensus problem} possess an invariant polytope that is efficiently computable \cite{Chevalier2015}.
We show in \cref{theo:hinvpoly} that if there is only one unstable cycle and its length is one then the optimal entropy is $\log_2(m)$ and it is attained by a hierarchy of \DBA{} lifts.

\begin{lemma}[{\cite[Theorem~2(v)]{szczyrba2015analytic}}]
  \label{theo:fibo}
  Given a set of $m$ symbols including symbol $l$, let $F_t^{(k)}(m-1)$ be the number of words of $t$ symbols that do not contain $k$ consecutive $l$'s.
  Let
  \begin{equation}
    \label{eq:Phi}
    \Phi^{(k)}(m-1) \triangleq \lim_{t \to \infty} [F_t^{(k)}(m-1)]^{1/t}.
  \end{equation}
  For any positive integer $m$, $\lim_{k \to \infty} \Phi^{(k)}(m-1) = m$.
\end{lemma}

\begin{theorem}
  \label{theo:hinvpoly}
  Given a switched system that possess an invariant polytope and the only unstable cycle of the switched system is $l$ for a given symbol $l \in \{1, \ldots, m\}$.
  The optimal value of \cref{eq:prob} is $h^* = \log_2(m)$ where $m$ is the number of matrices.

  \begin{myproof}
    Let $\Lang_k$ be the regular language allowing any word that does not contain $k$ consecutive $l$'s.
    By \cref{theo:fibo}, the entropy of $\Lang_k$ is given by $h(\Lang_k) = \log_2[\Phi^{(k)}(m-1)]$ where $\Phi$ is defined in \eqref{eq:Phi}
    and $\lim_{k \to \infty} h(\Lang_k) = \log_2 m$.
    As $\Lang_k$ is feasible for any $k$, $h^* \geq \lim_{k \to \infty} h(\Lang_k) = \log_2(m)$.
  \end{myproof}
\end{theorem}

%To prove this theorem, we need the following.
%\begin{lemma}[{\cite[Theorem~4.3.6]{Lind1995}}]
%  \label{lemma:cycle}
%  Given a regular language $\Lang$ recognized by an right-resolving automaton $\Autom$,
%  the following holds
%  \[ h(\Lang) = \lim_{k \to \infty} \frac{1}{k} \log_2|\Cycles|, \]
%  where $\Cycles$ represents the number of cycles of length $k$.
%
%\ifreport
%	\begin{myproof}
%	   We provide an alternative proof to the one in \cite[Theorem~4.2.6]{Lind1995}.
%	   As $\Cycles \leq \Paths$ for all $k$, we have
%	   \[ \lim_{k \to \infty} \frac{1}{k} \log_2|\Cycles| \leq h(\Lang) \]
%	   As $\Autom$ is right resolving, $|\Cycles| = \trace(\Adj^k)$.
%	   \claudio{Is the trace always defined for this kind of adjacency matrix? Suppose we have a single cycle with length $k$. Then, every $n$ that is not multiple of $k$ will yield $\trace(\Adj^n)=0$ and every $n$ multiple of $k$ will yield $\trace(\Adj^n)=k$. Thus the value of $\lim_{k \to \infty} \frac{1}{k} \log_2|\Cycles|$ never converges. What am I missing?}
%	   Let $\lambda_1, \ldots, \lambda_n$ be the eigenvalues of the adjacency matrix of $\Autom$ with $|\lambda_1| \geq \ldots \geq |\lambda_n|$,
%	   we have
%	   \[ \trace(\Adj^k) = \sum_{i=1}^n \lambda_i^k = |\lambda_1|^k \sum_{i=1}^n (\lambda_i/|\lambda_1|)^k \]
%	   hence
%	   \[ \frac{1}{k}\log_2\trace(\Adj^k) = \log_2 |\lambda_1| + \frac{1}{k} \log_2 \sum_{i=1}^n (\lambda_i/|\lambda_1|)^k. \]
%	   We have $\frac{1}{k} \log_2 \sum_{i=1}^n (\lambda_i/|\lambda_1|)^k = 0$ and $|\lambda_1| = \rho(\Adj)$.
%	   Since the automaton is right-resolving, $\rho(\Adj) = 2^{h(\Lang)}$.
%	   \benoit{We need to mention the Perron-Frobenius Theorem for it to be correct.}
%	 \end{myproof}
%\fi
%\end{lemma}
%
%\begin{lemma}
%  \label{lem:hleq}
%  Under \cref{as:1cycle},
%  the optimal value $h^*$ of \cref{eq:prob} satisfies $h^* \leq \log_2(m)$
%  where $m$ is the number of matrices.
%
%  \begin{myproof}
%    If \(h^* > \log_2(m)\), it means that there exist a regular language $\Lang$ with right-resolving automaton $\Autom$
%    \ifreport
%	  (we can suppose that it is right-resolving as every regular language is recognized by a right-resolving automaton)
%	\fi
%    such that $h(\Lang) > \log_2(m)$.
%    By \cref{lemma:cycle}, there exists $k$ such that
%    $|\Cycles| > 2^m$
%    \claudio{Not sure of the above step. In the worst case, $|\Cycles| = \trace(\Adj^k) = \sum_{i=1}^n \lambda_i^k \leq n m^k$. How do we go from that to the conclusion that there is a shared cycle?}
%    which means that there is a $c$ which is a cycle for both $\Lang$ and $\tilde{\Lang}$.
%    As it is a cycle in $\tilde{\Lang}$, it is unstable, which is absurd as $\Lang$ is admissible by \eqref{eq:admissible}.
%  \end{myproof}
%\end{lemma}
%
%\begin{lemma}[{\cite[Theorem~2(v)]{szczyrba2015analytic}}]
%  \label{theo:fibo}
%  Given an alphabet of $m$ letters including letter $l$, let $F_t^{(k)}(m-1)$ be the number of words of $t$ letters that do not contain $k$ consecutive $l$'s.
%  Let
%  \begin{equation}
%    \label{eq:Phi}
%    \Phi^{(k)}(m-1) \triangleq \lim_{t \to \infty} [F_t^{(k)}(m-1)]^{1/t}.
%  \end{equation}
%  For any positive integer $m$, $\lim_{k \to \infty} \Phi^{(k)}(m-1) = m$.
%\end{lemma}
%%\claudio{Nicely found, this result! Shouldn't it be a lemma here?}
%
%\begin{lemma}
%  \label{lem:hgeq}
%  If a polytope $P$ is invariant for a switched system and
%  $\tilde{\Lang}_P$ is the set of all repetitions of a letter $l$,
%  then %the optimal value $h^*$ of \cref{eq:prob} satisfies
%  \begin{equation*}
%    h^* \geq \log_2(m) - h(\tilde{\Lang}_P).
%  \end{equation*}
%  %where $m$ is the number of matrices.
%
%  \begin{myproof}
%    The number of words of $\tilde{\Lang}_P$ is 1 for any length $t$ so $h(\tilde{\Lang}_P) = 0$.
%    Let $\Lang_k$ be the regular language allowing any word that does not contain $k$ consecutive $l$'s.
%    By \cref{theo:fibo}, the entropy of $\Lang_k$ is given by $h(\Lang_k) = \log_2[\Phi^{(k)}(m-1)]$ where $\Phi$ is defined in \eqref{eq:Phi}
%    and $\lim_{k \to \infty} h(\Lang_k) = \log_2 m$.
%    As $\Lang_k$ is feasible for any $k$, $h^* \geq \lim_{k \to \infty} h(\Lang_k) = \log_2(m)$.
%  \end{myproof}
%\end{lemma}
%
%\begin{detachedproof}{\cref{theo:hinvpoly}}
%  By \cref{lem:hleq} and \cref{lem:hgeq}.
%\end{detachedproof}

\ifreport
  We conjecture the following generalization of \cref{theo:hinvpoly}.
  \cref{lem:hleq} already provides the first part of the proof of this conjecture but
  the generalization of \cref{lem:hgeq} still needs to be proven.
  
  \begin{conjecture}
    \label{conj:hinvpoly}
    If a polytope $P$ is invariant for a switched system,
    and $\tilde{\Lang}$ is as defined above, then the optimal value of \cref{eq:prob} is
    \begin{equation}
      h^* = \log_2(m) - h(\tilde{\Lang}),
    \end{equation}
    where $m$ is the number of matrices.
  \end{conjecture}
\fi


==> notes.tex <==
\section{Notes}

\begin{theorem}
$\rho(S) = \limsup_{t \to \infty} \jsr_t(S)$ exists, and
$\rho(S) = \inf \jsr_t(S)$.
\end{theorem}
\begin{myproof}

This proof is adapted from \cite{Jungers2009}.

Let us define the sequence $\set{ t \cdot \log \jsr_t(S) }_t$ which, for any $t \geq 0$, we have
$$\log \pargroup{\jsr_t(S)}^t  \Leftrightarrow$$
$$\log \pargroup{\sup_{A \in \Lambda^t} \norm{A}^\frac{1}{t}}^t \Leftrightarrow$$
$$\log \pargroup{\sup_{A \in \Lambda^t} \norm{A}}$$

Suppose $A = A_{n-1} \ldots A_{m} A_{m-1} \ldots A_{0} \in \Lambda^{n+m}$ and that
$\norm{A} = \sup_{B \in \Lambda^{n+m}} \norm{B}$.

Furthermore, from the automata structure, we know that \claudio{we probably need to show this}
$A_{n-1} \ldots A_{m} \in \Lambda^n$ and that
$A_{m-1} \ldots A_{0} \in \Lambda^m$.

By submultiplicativity, we have
$$ \norm{A_{n-1} \ldots A_{m} A_{m-1} \ldots A_{0}} \leq \norm{A_{n-1} \ldots A_{m}} \norm{A_{m-1} \ldots A_{0}} $$
and,
since
$$\norm{A_{n-1} \ldots A_{m}} \leq \sup_{B_{n-1} \ldots B_{m} \in \Lambda^n} \norm{B}$$
and
$$\norm{A_{m-1} \ldots A_{0}} \leq \sup_{B_{m-1} \ldots B_{0} \in \Lambda^m} \norm{B}$$
we conclude,
$$ \sup_{A \in \Lambda^{n+m}} \norm{A} \leq \pargroup{\sup_{A \in \Lambda^{n}} \norm{A}} \pargroup{\sup_{A \in \Lambda^{m}} \norm{A}} $$
and
\begin{aligneq}\label{eq:subadditivity}
\log \pargroup{\sup_{A \in \Lambda^{n+m}} \norm{A}} \leq \log \pargroup{\sup_{A \in \Lambda^{n}} \norm{A}} + \log \pargroup{\sup_{A \in \Lambda^{m}} \norm{A}}
\end{aligneq}

By Fekete's lemma,
$$ \lim_{t \to \infty} \frac{1}{t} \log \pargroup{\sup_{A \in \Lambda^t} \norm{A}} = \lim_{t \to \infty} \log \jsr_t(S) $$
exists, and
\begin{aligneq}\label{eq:fekete_lemma_applied}
\lim_{t \to \infty} \frac{1}{t} \log \pargroup{\sup_{A \in \Lambda^t} \norm{A}} = \inf \frac{1}{t} \log \pargroup{\sup_{A \in \Lambda^t} \norm{A}} = \inf \log \jsr_t(S)
\end{aligneq}

Which implies that
$$ \rho(S) = \inf \jsr_t(S) $$

\claudio{
Intuitively, it makes sense that we can now write $ \limsup_{t \to \infty} \jsr_t(S) = \lim_{t \to \infty} \jsr_t(S) $, but I'm missing the formal argument\ldots
}

\end{myproof}

\begin{theorem}
For any $m>0$, we have an upper bound on $\rho(S)$, given by
\begin{aligneq}\label{eq:upper_bound}
\rho(S) = \inf \jsr_t(S) \leq  \jsr_m(S)
\end{aligneq}
\end{theorem}

\begin{myproof}

\claudio{The argument below is adapted from \cite{Theys2005}.}

Suppose that, for a given $m>1$, $\jsr_m < 1$.
Then, from \cref{eq:upper_bound} we know that $\rho(S)<1$.
And, from the definition in \cref{eq:cjsr},
$$
\lim_{t \to \infty} \jsr_t(S) < 1
$$
Which means that there is a $t$ and $\gamma$, such that
$$ 0 \geq \jsr_t(S) = \gamma < \frac{\gamma + 1}{2} < 1  $$
the same as
$$ 0 \geq \sup_{A \in \Lambda^t} \norm{A}^\frac{1}{t} < \frac{\gamma + 1}{2} < 1 $$
$$ 0 \geq \sup_{A \in \Lambda^t} \norm{A} < \pargroup{\frac{\gamma + 1}{2}}^t < 1 $$

From the fact that
$$\lim_{t \to \infty} \pargroup{\frac{\gamma + 1}{2}}^t = 0$$
we have
$$\lim_{t \to \infty} \sup_{A \in \Lambda^t} \norm{A} = 0$$
and, for any $x_0$ and any $A \in \Lambda^t$, we have
$$\norm{x_{t}} \leq \norm{A} \norm{x_0}$$
Hence,
$$\lim_{t \to \infty} \norm{x_{t}} = 0$$

\end{myproof}


\begin{theorem}\label{th:cjsr_lower_bound}
$$\rho_t(S) \leq \rho(S)$$
\end{theorem}
\begin{myproof}
Let $k>0$.
Then
$$\rho_k(S) = \sup_{A \in \Lambda^k} \rho(A)^\frac{1}{k}$$
Now let $m>0$ in
$$\rho_k(S) = \sup_{A \in \Lambda^k} \rho(A)^\frac{m}{mk}$$
By the property $\rho(A)^m = \rho(A^m)$, we have
$$\rho_k(S) = \sup_{A \in \Lambda^k} \rho(A^m)^\frac{1}{mk}$$

\claudio{Can we prove this theorem for the following definition?}
$$\rho_k(S) = \sup_{\color{red} A \in \Lambda^k \wedge \forall n, A^n \in \Lambda^{nk}} \rho(A)^\frac{1}{k}$$
\claudio{And is it worth it? It all boils down to the case of whether it is worth getting an automaton as the one in \cref{fig:weakly_connected_automaton}}

Now note that
$$\rho_{mk}(S) = \sup_{A \in \Lambda^{mk}} \rho(A)^\frac{1}{mk}$$
includes many more accepted product matrices than $\rho_k(S)$.
Since it is a supremum, we have
$$ \rho_k(S) \leq \rho_{mk}(S) $$

Furthermore, taking the limit, we have
$$ \rho_{mk}(S) \leq \limsup_{m \to \infty} \rho_{mk}(S) $$

Now, the limit
$$ \rho(S) =  \limsup_{t \to \infty} \rho_{t}(S) $$
includes all the sequences of the limit
$$
\limsup_{m \to \infty} \rho_{mk}(S)
$$
and therefore,
$$ \limsup_{m \to \infty} \rho_{mk}(S) \leq \rho(S) $$

\end{myproof}

\begin{theorem}
$$\rho(S) \leq \jsr(S)$$
\end{theorem}
\begin{myproof}
\claudio{To do. Adapt from \cite{Theys2005}}
\end{myproof}


\begin{theorem}
From \cite{Legat2016}.
If there is a strictly positive homogeneous polynomial $p_v(x)$ of degree $2d$ for each $v \in V$ such that
\begin{aligneq}\label{eq:nice_poly}
p_v(A_\sigma x) \leq \gamma^{2d} p_u(x)
\end{aligneq}
holds for each edge $(u,v,\sigma)$ in the automaton.
Then $\rho(S) \leq \gamma$.
\end{theorem}
\begin{myproof}
We assume all matrix norms used here are matrix induced norms.
From the assumptions, we can find an upper and lower bounds to the polynomial $p_v(x)$ for all $x$ and each $v$.
That is, there exists $0 < \alpha_v \leq \beta_v$ such that
\begin{aligneq}\label{eq:bounds_poly}
\alpha_v \norm{x}^{2d} \leq p_v(x) \leq \beta_v \norm{x}^{2d}
\end{aligneq}
Consider a path $\sigma_1, \sigma_2, \ldots , \sigma_k$ with $k$ symbols and the intermediary $k+1$ nodes as $v_0, v_1, \ldots , v_k$.
For any $x_0 \in \setreal^n$, let $x_i = A_{\sigma_i} A_{\sigma_{i-1}} \ldots A_{\sigma_1} x_0$, for $i=1,\ldots,k$.
\cref{eq:bounds_poly}, for $x_k$, can be written as
\begin{aligneq}\label{eq:bounds_poly_expansion}
\alpha_v \norm{x_k}^{2d} &\leq p_v(x_k) \Leftrightarrow \\
\alpha_v \norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0}^{2d} &\leq p_v(A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0) \Leftrightarrow \\
\alpha_v^\frac{1}{2d} \norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0} &\leq p_v(A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0)^\frac{1}{2d} \Leftrightarrow \\
\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0} &\leq \alpha_v^{-\frac{1}{2d}} p_v(A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0)^\frac{1}{2d}
\end{aligneq}

\cref{eq:nice_poly} implies that
$$ p_v(A_\sigma x_{k-1})^\frac{1}{2d} \leq \gamma p_u(x_{k-1})^\frac{1}{2d} $$

Then, \cref{eq:bounds_poly_expansion} can be written as:
\begin{aligneq}\label{eq:bounds_poly_expansion}
\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0} &\leq \alpha_v^{-\frac{1}{2d}} p_v(A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0)^\frac{1}{2d} \\
							&\leq \alpha_v^{-\frac{1}{2d}} \gamma p_v(A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0)^\frac{1}{2d} \\
							&\leq \alpha_v^{-\frac{1}{2d}} \gamma^2 p_v(A_{\sigma_{k-2}} \ldots A_{\sigma_1} x_0)^\frac{1}{2d} \\
							& \ldots \\
							&\leq \alpha_v^{-\frac{1}{2d}} \gamma^k p_v(x_0)^\frac{1}{2d}
\end{aligneq}

From \cref{eq:bounds_poly}, we know that
$$ p_v(x_0)^\frac{1}{2d} \leq \beta_{v_0}^\frac{1}{2d} \norm{x_0} $$
therefore,
$$ \alpha_v^{-\frac{1}{2d}} \gamma^k p_v(x_0)^\frac{1}{2d} \leq \alpha_v^{-\frac{1}{2d}} \gamma^k \beta_{v_0}^\frac{1}{2d} \norm{x_0} $$
So we can write \cref{eq:bounds_poly_expansion} as:
\begin{aligneq}
\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0} &\leq \pargroup{\frac{\beta_{v_0}}{\alpha_v}}^{\frac{1}{2d}} \gamma^k \norm{x_0} \Leftrightarrow \\
\frac{\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0}}{\norm{x_0}} &\leq \pargroup{\frac{\beta_{v_0}}{\alpha_v}}^{\frac{1}{2d}} \gamma^k
\end{aligneq}

\claudio{Notice that the above equation differs from the one in \cite{Legat2016} in the element $\alpha_v$.
The expression in \cite{Legat2016} is as follows:}
\begin{aligneq}
\frac{\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0}}{\norm{x_0}} &\leq \pargroup{\frac{\color{red}\beta_{v_k}}{\color{red}\alpha_{v_0}}}^{\frac{1}{2d}} \gamma^k
\end{aligneq}

Since $\norm{\cdot}$ is a matrix induced norm, we have
\begin{aligneq}
\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1}} =\\
		&= \sup_{x \neq 0} \frac{\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x}}{\norm{x}} \\
		&= \max_{\norm{x} = 1} \norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x}
\end{aligneq}
which, due to the supremum, we have
\begin{aligneq}
\frac{\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x_0}}{\norm{x_0}} \leq \norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1}}
\end{aligneq}
Moreover, since the above reasoning applies to any $x_0$, we can pick the $x$ such that
\begin{aligneq}\label{eq:max_x_chosen}
\frac{\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1} x}}{\norm{x}} = \norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1}}
\end{aligneq}

And so, for such $x$, we can conclude:
\begin{aligneq}
\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1}} \leq \pargroup{\frac{\beta_v}{\alpha_v}}^{\frac{1}{2d}} \gamma^k \leq \pargroup{\frac{\beta}{\alpha}}^{\frac{1}{2d}} \gamma^k
\end{aligneq}

Taking the $k$-th root, we have
\begin{aligneq}
\pargroup{\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1}}}^\frac{1}{k} \leq \pargroup{\frac{\beta_v}{\alpha_v}^{\frac{1}{2d}}}^\frac{1}{k} \gamma \leq \pargroup{\frac{\beta}{\alpha}^{\frac{1}{2d}}}^\frac{1}{k} \gamma
\end{aligneq}

To take the limit $k \to \infty$, one must note that for $k + 1$,
we must pick a different $x$ than the one chosen for $k$.
Such $x$ is guaranteed to exist and satisfies \cref{eq:max_x_chosen}.
Hence, the limit can be safely taken, and we get:
\begin{aligneq}\label{eq:limit_k}
\norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1}}^\frac{1}{k} &\leq \pargroup{\frac{\beta}{\alpha}^{\frac{1}{2d}}}^\frac{1}{k} \gamma \Leftrightarrow \\
\lim_{k\to\infty} \norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1}}^\frac{1}{k} &\leq \gamma
\end{aligneq}

Since $\rho(S) = \lim_{k \to \infty} \max \set{ \norm{A_{\sigma_k} A_{\sigma_{k-1}} \ldots A_{\sigma_1}}^\frac{1}{k} }$,
and since \cref{eq:limit_k} applies to any path of length $k$, we can pick the maximum path and thus conclude the proof:
$$ \rho(S) \leq \gamma $$

\end{myproof}


\section{Notes on Problem Formulation}

\claudio{What are the assumptions that we make about the constraint automaton?
Does it have to be strongly connected? \cite{Philippe2016} assumes that the automaton is strongly connected by I think we don't need this assumption.
Suppose we have an automaton as in \cref{fig:weakly_connected_automaton}, which is not strongly connected.
It can never be the case that the path $cbade$ causes the system to be unstable, because it cannot be repeated.
It must either be the cycle $cba$ or $e$ that makes the system unstable.
So, I presume, the path $cbade$ can never be returned by the CJSR tool.
Since we will be dealing with infinitely long paths, we must at least assume that $\mathbf{G}$ has at least one cycle.
}

\begin{figure}[tbh]
\begin{center}
  \includegraphics[width=0.3\textwidth]{weakly_connected_automaton}
  \caption{figureCaption}
  \label{fig:weakly_connected_automaton}
\end{center}
\end{figure}


Our approach assumes that only one such sequence can be found at any time.
If there is one such sequence, it represents a cycle, and then there can be an infinite number of sequences that make the system unstable.
To see this, suppose that the algorithm returns a cycle $A_\sigma(k), \ldots, A_\sigma(l)$, for some $0 \leq  k \leq l$.
Then, any other (infinite) path in the graph that ends with $\pargroup{A_\sigma(k), \ldots, A_\sigma(l)}^*$ \claudio{Is it worth it to use ( and introduce) regular language notation?} will also make the system unstable (because the instability definition holds for any $x$).
However, as the dwell time approaches show \claudio{Citations to related work}, it may be the case that there is a cycle $A_\sigma(g), \ldots, A_\sigma(k), \ldots, A_\sigma(l), \ldots, A_\sigma(m)$, with $0 \leq g \leq k \leq l \leq m $, of which $A_\sigma(k), \ldots, A_\sigma(l)$ is a sub-cycle, that does not make the system unstable.
For example, in the adaptive numerical method example, with constraint automaton as in \cref{fig:order_adaptive_method}, $\tilde{A}_1$ satisfies $\rho(\tilde{A}_1) > 1$ (and therefore $\rho_1(S) > 1$), but $\rho(\tilde{A}_2 \cdot \tilde{A}_1) < 1$.

\claudio{We need to provide values for matrix $A$ of the adaptive numerical example, in order to make these examples concrete. Ideally, these should be values which we can compute with the brute force method, so that we can show their upper and lower bounds for finite products.}

Once a cycle $A_\sigma(k), \ldots, A_\sigma(l)$, for some $0 \leq  k \leq l$, that makes the system unstable has been identified, a new constraint automaton $\mathbf{G}$ must be created that does not accept sequences of the form $(A_\sigma(k), \ldots, A_\sigma(l))^*$.
A straightforward way of doing this is to ``remove'' one of the edges in $\set{(v,u,\sigma(i)) : i=k,\ldots,l}$.
\claudio{Explain this formally.}
Then, compute $\rho(S')$, where $S'$ is the new switched system constrained by $\mathbf{G'}$.
If $\rho(S')>1$ holds, then repeat the process.
Otherwise, since $\Mats$ is bounded, the system is stable. \claudio{I think this is proven in \cite{Dai2012}}.
\claudio{We purposefully omit details here (such as, does the algorithm terminate? What happens to the structure of the automata as it gets its edges remove, etc\ldots), as this is only the problem formulation section.}

If the procedure sketched here is applied to the adaptive solver example, we get the automaton shown in \cref{fig:order_adaptive_method_stable}.

\begin{figure}[tbh]
\begin{center}
  \includegraphics[width=0.3\textwidth]{order_adaptive_method_stable}
  \caption{figureCaption}
  \label{fig:order_adaptive_method_stable}
\end{center}
\end{figure}

A sensible question, and part of out contribution, regarding the algorithm described above is:
\emph{Which edge should be removed to break an unstable cycle?} \claudio{we should probably define the term ``unstable cycle''}

Furthermore, it is easy to see that any sequence of the form $(\tilde{A}_1)^{r}, (\tilde{A}_2)^s$ with $r \geq 0$ and $s \geq 0$ is also forbidden.
This is too restrictive since, for $r = s$, the sequence does not make the system unstable.
To see why, first note that $\tilde{A}_1 \cdot \tilde{A}_2 = \tilde{A}_2 \cdot \tilde{A}_1$.
Hence, we can write the matrix product induced by the sequence as
$$
\tilde{A}_1^r \cdot \tilde{A}_2^r = \pargroup{\tilde{A}_1 \cdot \tilde{A}_2}^r
$$
And $\rho(\pargroup{\tilde{A}_1 \cdot \tilde{A}_2}^r)^\frac{1}{2r} = \rho(\pargroup{\tilde{A}_1 \cdot \tilde{A}_2})^\frac{1}{2} < 1$.
which tells us that any one of these sequences alone could not make the system unstable.

We therefore propose to explore \emph{how to forbid the sequences, and only those, that make the system unstable.}


\section{Notes on Stabilization of Unconstrained}


Consider an unconstrained switched system with matrices $\Sigma = \set{A_1, \ldots, A_N}$.
This system can be seen as a constrained switched system $S = (\mathbf{G}, \Sigma)$, whose automaton $\mathbf{G}$ has a single node, and an edge per matrix in $\Sigma$.
The language accepted by $S$ is $\Sigma^* = \bigcup_{t}^\infty \Sigma^t$ and the infinitely long sequences are $\Sigma^\infty$.
An example is shown in \cref{fig:unconstrained_automaton}.

\begin{figure}[tbh]
\begin{center}
  \includegraphics[width=0.3\textwidth]{unconstrained_automaton}
  \caption{Caption}
  \label{fig:unconstrained_automaton}
\end{center}
\end{figure}

Removing an edge $(v,v,\sigma)$ in $\mathbf{G}$ amounts to forbidding the use of matrix $A_\sigma \in \Sigma$, which means that the infinitely long sequence set becomes $\pargroup{\Sigma \setminus \set{A_\sigma}}^\infty$ whereas the intention was $\Sigma^\infty \setminus \set{A_\sigma^\infty}$. \claudio{we should give more prominence to infinitely long sequences, since those are the ones we are looking at for stability.}.
This is too conservative.

\subsubsection{Product Lift}

One way of doing this is, given an $m > 0$, enumerate all sequences of length $m$ that are accepted by $S$, and create a constrained switched system $S$ with a single node automaton, and an edge corresponding to each sequence.
This is exemplified in \cref{fig:path_expanded_unconstrained_automata}.
The new switched system represents $m$ steps of the original switched system but, from the point of view of stability, the infinitely long sequences are the same. \claudio{How do we formalize this?}
The accepted infinitely long sequences \claudio{should we call these ``asymptotic sequences''} are $\Lambda^\infty = \pargroup{\Sigma^m}^\infty = \Sigma^\infty$ \claudio{How do we show this formally?}.

\begin{figure}[tbh]
\begin{center}
  \includegraphics[width=0.3\textwidth]{path_expanded_unconstrained_automata}
  \caption{A flower.}
  \label{fig:path_expanded_unconstrained_automata}
\end{center}
\end{figure}

Suppose we remove edge $(v,v,\sigma(0)\ldots\sigma(m-1))$.
Then, the new set of infinitely long sequences is $\pargroup{\Sigma^m \setminus \set{A_{\sigma(m)} \ldots A_{\sigma(0)}}}^\infty$.

\claudio{The ``proof'' bellow should be omitted.}

To see why this is less conservative, assume that edge $(v,v,\sigma(0)\ldots\sigma(m-1))$ needed to be removed because the cycle $(v,v,\sigma(0)\ldots\sigma(m-1))$ is unstable, that is, $\rho(A{_\sigma(m)} \ldots A_{\sigma(0)}) > 1$.
The case for larger cycles being unstable reduces to removing a single edge anyway, so we don't lose generality in this assumption.
Now, either there is at least one matrix $A_{\sigma(i)}$ in the product $A_{\sigma(m)} \ldots A_{\sigma(0)}$ that is unstable, or all matrices are stable.

In the first case, the procedure to find the unstable cycle in the original constraint system $S$ would have returned the cycle $A_{\sigma(i)}$, and the edge to be removed would be $(v,v, A_{\sigma(i)})$.

In the second case, the procedure to find the unstable cycle in the original constraint system $S$ would have returned the cycle $A_{\sigma(0)}, \ldots , A_{\sigma(m)}$, and an edge to be removed has to be chosen. \claudio{In this case, does the algorithm return the smallest such sequence? Or can there be a smaller subsequence that is unstable? Anyhow, this should not be hard to check, we just evaluate the spetral radius in all subsequences.}
Suppose that edge $(v,v, A_{\sigma(i)})$ is chosen. Notice that we don't loose generality is naming this edge $(v,v, A_{\sigma(i)})$, even if it is different than the edge to be removed in the first case. What matter is that $A_{\sigma(i)}$ appears in the product $A_{\sigma(m)} \ldots A_{\sigma(0)}$.

The set of infinitely long sequences for the transformed original system is $\Lambda^\infty = \pargroup{\Sigma \setminus \set{A_{\sigma(i)}}}^\infty$ whereas the set of infinitely long sequences for the transformed expanded system is $\Lambda'^\infty = \pargroup{\Sigma^m \setminus \set{A_{\sigma(m)} \ldots A_{\sigma(i)} \ldots A_{\sigma(0)}}}^\infty$.
Now, we just have to show that $\Lambda^\infty \subseteq \Lambda'^\infty$.

Given an infinitely long sequence $A_{s(0)}, A_{s(1)}, \ldots$ from $\Lambda^\infty$.
We know that $A_{\sigma(i)}$ does not take part in $A_{s(0)}, A_{s(1)}, \ldots$.
Hence, the sequence $A_{\sigma(0)}, \ldots, A_{\sigma(i)}, \ldots, A_{\sigma(m)}$ is not a subsequence of $A_{s(0)}, A_{s(1)}, \ldots$.
If we group $A_{s(0)}, A_{s(1)}, \ldots$ in groups of $m$ elements, if is easy to see that each group is a member of $\Sigma^m \setminus \set{A_{\sigma(m)} \ldots A_{\sigma(i)} \ldots A_{\sigma(0)}}$, which means that $A_{s(0)}, A_{s(1)}, \ldots$ is in $\Lambda'^\infty$.

\claudio{Ideally, the above ``proof'' must be made for increasing values of $m$. That is, so that $m$ is less conservative than $m+1$.}

\claudio{Apply this approach to the numerical example, and show how the resulting system is less conservative than the measure takn in the problem formulation.}

\section{General System Structure for Co-simulation}


Since the simulators only exchange outputs at times $t_i$ and $t_{i+1}$, the input $u_j$ has to be extrapolated in the interval $\brackets{t_i, t_{i+1}}$.
Without loss of generality\footnote{We could have considered extrapolations that depends on the derivatives (up to any order) of previous input points, but that would make the notation cumbersome.}, and for simplicity of notation, we assume that such extrapolation depends on the past $p+1$ inputs.
If this extrapolation can be represented \footnote{This representation can be computed for Lagrange and Taylor polynomials.} as
$\Phi(t)_j = E_j(t) \cdot \bar{u}_j$
where $E_j(t)$ is a function of time $t \in \brackets{t_i, t_{i+1}}$, and
$\bar{u}_j = \brackets{ u_j(t_i) \ldots u_j(t_{i-p})}^T$
is the extended input vector, then \cref{eq:linear_ode}
can be re-written to represent the unforced system being integrated by each simulator:
\begin{aligneq}\label{eq:linear_ode_unforced}
\vectorTwo{\dert{x}_j}{\dert{\bar{u}}_j} &= \vectorTwo{A_j & E_j(t)}{\mathbf{0} & \mathbf{0}} \cdot \vectorTwo{x_j}{\bar{u}_j}
\end{aligneq}

If the numerical method in use by each simulator can be represented as a matrix, such as the ones used in \cref{eq:adaptive_numerical_method}, then we can represent the multiple internal integration steps of \sys{eq:linear_ode_unforced}, performed by the simulator $S_j$ in the interval $t \in \brackets{t_i, t_{i+1}}$, as
\begin{aligneq}\label{eq:solver_internal_steps}
\vectorTwo{x_j(t_{i+1})}{\bar{u}_j(t_{i+1})} &= \tilde{A}^{k_j}_j \cdot \vectorTwo{x_j(t_i)}{\bar{u}_j}
\end{aligneq}
where, e.g., $\tilde{A}_j = I + \vectorTwo{A_j & E_j(t)}{\mathbf{0} & \mathbf{0}}$ for the Forward Euler method,
$k_j=(t_{i+1} - t_i)/h_j$ is the number of internal steps, and $0 < h_j \leq H$ is the internal fixed step size that divides $H$.

At the beginning of the co-simulation step $i$, we wish to compute $u_1(t_i) = y_2(t_i)$ and $u_2(t_i) = y_1(t_i)$.
This, together with \cref{eq:linear_ode}, gives,
\begin{aligneq}
u_1(t_i) &= C_2 \cdot x_2(t_i) \\
u_2(t_i) &= C_1 \cdot x_1(t_i) + D_1 C_2 \cdot x_2(t_i) \\
\end{aligneq}

Notice that, for $r = 1, \ldots p$,
\begin{aligneq}
u_1(t_{i-r}) &= C_2 \cdot x_2(t_{i-r}) \\
u_2(t_{i-r}) &= C_1 \cdot x_1(t_{i-r}) + D_1 C_2 \cdot x_2(t_{i-r}) \\
\end{aligneq}
Hence,
\begin{aligneq}\label{eq:io_couplings}
\bar{u}_1 &= \underbrace{\vectorFour{\mathbf{0} & C_2 & \mathbf{0} & \mathbf{0} & \ldots & \mathbf{0} & \mathbf{0}}%
						{\mathbf{0} & \mathbf{0} & \mathbf{0} & C_2  & \ldots & \mathbf{0} & \mathbf{0}}%
						{ &  &  & \vdots &  &  & }%
						{\mathbf{0} & \mathbf{0} & \mathbf{0} & \mathbf{0} & \ldots & \mathbf{0} & C_2}}_{U_1}
						\vectorSeven{x_1(t_i)}{x_2(t_i)}{x_1(t_{i-1})}{x_2(t_{i-1})}{\vdots}{x_1(t_{i-p})}{x_2(t_{i-p})} \\
\bar{u}_2 &= \underbrace{\vectorFour{C_1 & D_1 C_2 & \mathbf{0} & \mathbf{0} & \ldots & \mathbf{0} & \mathbf{0}}%
						{\mathbf{0} & \mathbf{0} & C_1 & D_1 C_2 & \ldots & \mathbf{0} & \mathbf{0}}%
						{ &  &  & \vdots &  &  & }%
						{\mathbf{0} & \mathbf{0} & \mathbf{0} & \mathbf{0} & \ldots & C_1 & D_1 C_2}}_{U_2}
						\vectorSeven{x_1(t_i)}{x_2(t_i)}{x_1(t_{i-1})}{x_2(t_{i-1})}{\vdots}{x_1(t_{i-p})}{x_2(t_{i-p})}
\end{aligneq}

Equations \ref{eq:linear_ode_unforced}, \ref{eq:solver_internal_steps}, and \ref{eq:io_couplings} can be used to represent the co-simulation steps as a linear discrete time system:
\begin{aligneq}\label{eq:co_simulation_dts}
\vectorTwo{x_1(t_{i+1})}{x_2(t_{i+1})} &=
	\vectorTwo{I & \mathbf{0} & \mathbf{0} & \mathbf{0}}{\mathbf{0} & \mathbf{0} & I & \mathbf{0}}
	\vectorTwo{\tilde{A}^{k_1}_1 & \mathbf{0}}{\mathbf{0} & \tilde{A}^{k_2}_2}
	\underbrace{
		\vectorFour{I & \mathbf{0}}{\mathbf{0} & C_2}{\mathbf{0} & I}{C_1 & D_1 \cdot C2}
		\vectorTwo{x_1(t_{i})}{x_2(t_{i})}
	}_{\vectorFour{x_1(t_{i})}{u_1(t_{i})}{\mathbf{0} & I}{C_1 & D_1 \cdot C2}}
\\
\vectorSeven{x_1(t_{i+1})}{x_2(t_{i+1})}{x_1(t_{i})}{x_2(t_{i})}{\vdots}{x_1(t_{i-p+1})}{x_2(t_{i-p+1})} &=
	\vectorSix{I 		  & \mathbf{0} & \mathbf{0} & \mathbf{0} & \ldots & \mathbf{0}}%
			  {\mathbf{0} & \mathbf{0} & I          & \mathbf{0} & \ldots & \mathbf{0}}%
			  {I          & \mathbf{0} & \mathbf{0} & \mathbf{0} & \ldots & \mathbf{0}}%
			  {\mathbf{0} & I 		   & \mathbf{0} & \mathbf{0} & \ldots & \mathbf{0}}%
			  {           &  		   & \ldots 	& 			 &		  &			  }%
			  {\mathbf{0} & \ldots 	   & \mathbf{0} & \mathbf{0} & \ldots & I		  }%
	\vectorSeven{\tilde{A}^{k_1}_1 & \mathbf{0} & \ldots & \mathbf{0}}%
				{\mathbf{0} & \tilde{A}^{k_2}_2 & \ldots & \mathbf{0}}%
				{I & \mathbf{0} & \ldots & \mathbf{0}}%
				{\mathbf{0} & I & \ldots & \mathbf{0}}%
				{ &  & \ldots & }%
				{\mathbf{0} & \ldots & I & \mathbf{0}}%
				{\mathbf{0} & \ldots & \mathbf{0} & I}
	\vectorSeven{I & \mathbf{0} & \ldots & \mathbf{0}}%
				{  &  U_1 &     &  }%
				{\mathbf{0} & I & \ldots & \mathbf{0}}%
				{  &  U_2  &    &  }%
				{I & \mathbf{0} & \ldots & \mathbf{0}}%
				{\mathbf{0} & I & \ldots & \mathbf{0}}%
				{\mathbf{0} & \ldots & I & \mathbf{0}}
	\vectorSeven{x_1(t_i)}{x_2(t_i)}{x_1(t_{i-1})}{x_2(t_{i-1})}{\vdots}{x_1(t_{i-p})}{x_2(t_{i-p})}
\end{aligneq}



